Agnostic learning with unknown utilities

Traditional learning approaches for classification implicitly assume that each mistake has the same cost. In many real-world problems though, the utility of a decision depends on the underlying context $x$ and decision $y$. However, directly incorporating these utilities into the learning objective is often infeasible since these can be quite complex and difficult for humans to specify. We formally study this as agnostic learning with unknown utilities: given a dataset $S = \{x_1, \ldots, x_n\}$ where each data point $x_i \sim \mathcal{D}$, the objective of the learner is to output a function $f$ in some class of decision functions $\mathcal{F}$ with small excess risk. This risk measures the performance of the output predictor $f$ with respect to the best predictor in the class $\mathcal{F}$ on the unknown underlying utility $u^*$. This utility $u^*$ is not assumed to have any specific structure. This raises an interesting question whether learning is even possible in our setup, given that obtaining a generalizable estimate of utility $u^*$ might not be possible from finitely many samples. Surprisingly, we show that estimating the utilities of only the sampled points~$S$ suffices to learn a decision function which generalizes well. We study mechanisms for eliciting information which allow a learner to estimate the utilities $u^*$ on the set $S$. We introduce a family of elicitation mechanisms by generalizing comparisons, called the $k$-comparison oracle, which enables the learner to ask for comparisons across $k$ different inputs $x$ at once. We show that the excess risk in our agnostic learning framework decreases at a rate of $O\left(\frac{1}{k} \right)$. This result brings out an interesting accuracy-elicitation trade-off -- as the order $k$ of the oracle increases, the comparative queries become harder to elicit from humans but allow for more accurate learning.

==> pop-analysis.tex <==
%!TEX root = reward-main-v2.tex
\section{Population-level bounds}
We begin with a study of our problem at the population level where we assume that the learner has access to the underlying distribution $\xdist$. The main objective is to provide an information-theoretic characterization of the error $\gap(\f, \F)$ without any constraints on the number of orcale calls.

Let $\simplex_\F$ and $\simplex_\uclass$ represent the set of probability distributions over the function class $\F$ and utility functions $\uclass$ respectively. Further, denote the set of all possible $\kor$-queries by
\begin{align*}
  \qset_\kor = \{\query = (\bx, \by_1, \by_2) \; | \; \bx \in \X^\kor, \by_1 \in \Y^\kor, \text{ and } \by_2 \in \Y^\kor\}.
\end{align*}
Further, for any $\kor$-comparison oracle $\oracle_\kor^{\u} $, let us represent the corresponding response set by
\begin{align*}
  \rset_{\kor}^\u = \{ (\query, \res) \;|\; \query \in \qset_\kor\},
\end{align*}
where $\res \in [0,1]$ is the probability that the oracle $\oracle_\kor^\u$ will output $1$ for a query $\query \in \qset_\kor$. Given this above setup, we define a notion of consistency of utility functions.
\begin{definition}
  A pair of utility functions $(\u, \u')$ are said to be $\kor$-consistent with respect to an oracle $\oracle_\kor$  if the sets $\rset_\kor^\u = \rset_\kor^{\u'}$, that is, the functions $\u$ and $\u'$ are indistinguishable with respect to $\oracle_\kor$.
\end{definition}
Given the above definition, we are interested in characterizing the instance-dependent minimax error
\begin{align*}
  \minmax(\oracle^{\utrue}_\kor, \F) \defn \pinf_{\ld \in \simplex_\F} \sup_{\u'\in\; \uclass_{\kor}^{\utrue}} \En_{\f \sim \ld}[ \gap(\f, \F; \u')]\;,
\end{align*}
where $\uclass_{\kor}^{\utrue} \subseteq \uclass$ represents the subset of utilities which are consistent with utility $\u$ with respect to oracle $\oracle_\kor$. Our first result is an upper bound on the above minimax value.

\begin{theorem}[Upper bound] For any distribution $\xdist$  over feature space $\X$, $\kor$-comparison orcale $\oracle_\kor^{\u}$ and function class $\F$, the minimax risk
  \begin{align*}
    \minmax(\oracle^{\u}_\kor, \F) \leq \sup_{\u_1, \u_2 \in\; \uclass_\kor^\u} \left( \util(\f_{\u_1};\u_1) - \util(\f_{\u_2};\u_1) \right),
  \end{align*}
  where $\f_{\bar{u}} \defn \argmax_{\f \in \F} \util(\f;\bar{\u})$ is the arg-maximizer with respect to utility $\bar{\u}$.
\end{theorem}
\begin{proof}
By an application of Sion's minimax theorem, we can write the minimax value $\minmax(\oracle^{\u}_\kor, \F)$ as
\begin{align*}
  \minmax(\oracle^{\utrue}_\kor, \F) &= \pinf_{\ld \in \simplex_\F} \sup_{\u'\in\; \uclass_{\kor}^{\u}} \En_{\f}[ \gap(\f, \F; \u')]\\
  &= \pinf_{\ld \in \simplex_\F} \sup_{\u'\in\; \uclass_{\kor}^{\u}} \sup_{\f' \in \F} \En_{\f} [\util(\f';\u') - \util(\f;\u')]\\
  &= \sup_{\ld \in \simplex_{\F \times \uclass_{\kor}^{\u}}} \pinf_{\f \in \F} \En_{(\f', \u')}\left[\util(\f';\u') - \util(\f;\u') \right],
\end{align*}
where $\simplex_{\F \times \uclass_{\kor}^{\u}}$ denotes the space of all distributions over the joint space $\F \times \uclass_{\kor}^{\u}$. Let us decompose the distribution $\ld = \ld_\u \cdot \ld_{\f|\u}$ where $\ld_\u$ represents the marginal distribution over the space $\uclass_{\kor}^{\u}$ and $\ld_{\f|\u}$ denotes the conditional distirbution of sampling a function $\f \in \F$ given utility function $\u$. Denote by $\f_u \defn \argmax_{\f\in \F}\util(\f;\u)$ and $\f_{p} \defn \argmax_{\f \in \F}\En_{\f \sim p}[\util(\f;\u)]$ as the maximizers for the corresponding utility functions. Then, the minimax value
\begin{align*}
  \minmax(\oracle^{\utrue}_\kor, \F)&= \sup_{\ld \in \simplex_{\F \times \uclass_{\kor}^{\u}}} \pinf_{\f \in \F} \En_{(\f', \u')}\left[\util(\f';\u') - \util(\f;\u') \right] \\
  &= \sup_{\ld_\u}\sup_{\ld_{\f|\u}} \pinf_{\f \in \F} \left(\En_{\u' \sim \ld_u} \En_{\f' \sim \ld_{\f|\u'}}\left[\util(\f';\u')\right] - \En_{\u' \sim \ld_u}\left[\util(\f;\u') \right]\right)\\
  &\stackrel{\1}{=} \sup_{\ld_\u}\sup_{\ld_{\f|\u}} \left(\En_{\u' \sim \ld_u} \En_{\f' \sim \ld_{\f|\u'}}\left[\util(\f';\u')\right] - \En_{\u' \sim \ld_u}\left[\util(\f_{\ld_u};\u') \right]\right)\\
  &\stackrel{\2}{=} \sup_{\ld_\u}\left( \En_{\u' \sim \ld_u} \left[\util(\f_{\u'};\u') - \util(\f_{\ld_u};\u') \right]\right),
\end{align*}
where the inequality $\1$ follows from the fact that $\f_{\ld_u}$ maximizes the expected utility with respect to $\ld_u$ and $\2$ follows by noting that the maximizing distribution $\ld_{\f|\u'} = \ind[\f = \f_{\u'}]$. Noting that $\f_{\ld_u}$ is the maximizer corresponding to the distribution $\ld_u$, we have,
\begin{align*}
  \minmax(\oracle^{\utrue}_\kor, \F)&= \sup_{\ld_\u}\left( \En_{\u' \sim \ld_u} \left[\util(\f_{\u'};\u') - \En_{\bar{\u}}[\util(\f_{\bar{\u}};\u')] + \En_{\bar{\u}}[\util(\f_{\bar{\u}};\u')] - \util(\f_{\ld_u};\u') \right]\right)\\
  &\leq \sup_{\ld_\u}\left( \En_{\u' \sim \ld_u} \left[\util(\f_{\u'};\u') - \En_{\bar{\u}}[\util(\f_{\bar{\u}};\u')] \right] \right)\\
  &\stackrel{\1}{\leq} \sup_{\u_1, \u_2 \in\; \uclass_\kor^\u} \left( \util(\f_{\u_1};\u_1) - \util(\f_{\u_2};\u_1) \right),
\end{align*}
where the inequality $\1$ follows by upper bounding the expected deviation with a worst-case deviation. This establishes the required claim.
\end{proof}
Having established the upper bound above, we now proceed to obtain a corresponding lower bound on the minimax risk in our next theorem.

\begin{theorem}[Lower Bound]
  For any distribution $\xdist$  over feature space $\X$, $\kor$-comparison oracle $\oracle_\kor^{\u}$ and function class $\F$, the minimax risk
    \begin{align*}
      \minmax(\oracle^{\u}_\kor, \F) \geq  \frac{1}{2} \cdot \sup_{\u_1, \u_2 \in\; \uclass_\kor^\u} \left( \util(\f_{\u_1};\u_1) - \util(\f_{\frac{\u_1+\u_2}{2}};\u_1) \right).
    \end{align*}
\end{theorem}
\begin{proof}
  Consider any two utility functions $\u_1, \u_2 \in \uclass_\kor^\u$ and let $\bar{u} = \frac{\u_1+\u_2}{2}$. We can then lower bound the minimax risk as
  \begin{align*}
    \minmax(\oracle^{\u}_\kor, \F) &\geq \inf_{\f \in \F} \left(\frac{1}{2}\gap(\f, \F;\u_1) + \frac{1}{2} \gap(\f, \F;\u_2) \right)\\
    &\geq \frac{1}{2}\gap(\f_{\bar{u}}, \F;\u_1) + \frac{1}{2} \gap(\f_{\bar{u}}, \F;\u_2)\\
    &\geq \frac{1}{2} \left(\util(\f_{\u_1};\u_1) - \util(\f_{\bar{\u}};\u_1) \right),
  \end{align*}
  where the last equality follows by noting that $\gap(\f_{\bar{u}}, \F;\u_2) \geq 0$. Since the above holds for any choice of $\u_1, \u_2$, the desired bound follows by taking a supremum over these values.
\end{proof}

